Exploring Semantic Consistency and Style Diversity for Domain Generalized Semantic Segmentation

Domain Generalized Semantic Segmentation (DGSS) seeks to utilize source domain data exclusively to enhance the generalization of semantic segmentation across unknown target domains. Prevailing studies predominantly concentrate on feature normalization and domain randomization, these approaches exhibit significant limitations. Feature normalization-based methods tend to confuse semantic features in the process of constraining the feature space distribution, resulting in classification misjudgment. Domain randomization-based methods frequently incorporate domain-irrelevant noise due to the uncontrollability of style transformations, resulting in segmentation ambiguity. To address these challenges, we introduce a novel framework, named SCSD for Semantic Consistency prediction and Style Diversity generalization. It comprises three pivotal components: Firstly, a Semantic Query Booster is designed to enhance the semantic awareness and discrimination capabilities of object queries in the mask decoder, enabling cross-domain semantic consistency prediction. Secondly, we develop a Text-Driven Style Transform module that utilizes domain difference text embeddings to controllably guide the style transformation of image features, thereby increasing inter-domain style diversity. Lastly, to prevent the collapse of similar domain feature spaces, we introduce a Style Synergy Optimization mechanism that fortifies the separation of inter-domain features and the aggregation of intra-domain features by synergistically weighting style contrastive loss and style aggregation loss. Extensive experiments demonstrate that the proposed SCSD significantly outperforms existing state-of-theart methods. Notably, SCSD trained on GTAV achieved an average of 49.11 mIoU on the four unseen domain datasets, surpassing the previous state-of-the-art method by +4.08 mIoU. Code is available at https://github.com/nhw649/SCSD.

==> section/exp_tab/table_abl_param.tex <==
\begin{table}[t]
    \begin{center}
        \begin{adjustbox}{max width=1.0\linewidth}
            \begin{tabular}{ccc}
                \begin{subtable}[t]{0.5\linewidth}
                    \centering
                    \begin{tabular}{ll|c}
                        \toprule
                         $\alpha$ & $\beta$ & $Avg.$ \\
                        \midrule
                        - & - & 21.1 \\
                        0.7 & 0.7 & 20.3 \\
                        0.8 & 0.7 & 20.4 \\
                        0.9 & 0.7 & 21.1 \\
                        0.9 & 0.8 & 21.5 \\
                        0.9 & 0.85 & 21.6 \\
                        0.9 & 0.9 & 20.1 \\
                        \bottomrule
                    \end{tabular}
                    \caption{Different mask quality threshold $m_t$ and class quality threshold $c_t$ in DDTF.}                    
                \end{subtable} &
                \begin{subtable}[t]{0.3\linewidth}
                    \centering
                    \begin{tabular}{l|c}
                        \toprule
                         $w_l$ & $Avg.$ \\
                        \midrule
                        0.5 & 19.9 \\
                        0.7 & 20.0 \\                        
                        0.9 & 20.0 \\
                        0.99 & 20.2 \\
                        0.999 & 21.0 \\
                        0.9996 & 21.6 \\
                        0.9999 & 19.1 \\
                        \bottomrule
                    \end{tabular}
                    \caption{Different EMA rate $\alpha$.}
                \end{subtable} &
                \begin{subtable}[t]{0.3\linewidth}
                    \centering
                    \begin{tabular}{l|c}
                        \toprule
                         $\lambda$ & $Avg.$ \\
                        \midrule
                        0.5 & 21.1 \\
                        1 & 21.6 \\
                        2 & 18.6 \\
                        4 & 10.0 \\
                        8 & 6.6 \\
                        \bottomrule
                    \end{tabular}
                    \caption{Different weight $\lambda$ for the unsupervised loss $\mathcal{L}_\mathrm{unsup}$.}
                \end{subtable}
            \end{tabular}
        \end{adjustbox}
    \end{center}
    \caption{Hyper-parameters in Our SCSD.}
    \label{table_abalation_hyper-parameters}
\end{table}

==> section/exp_tab/table_acdc_r50x16.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{max width=0.47\textwidth}
\begin{tabular}{c|ccccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{5}{c}{Trained on GTAV (G)} \\
    \cmidrule(lr){2-6}
    % \midrule
    & $\rightarrow$ AN & $\rightarrow$ AS & $\rightarrow$ AR & $\rightarrow$ AF & Avg.\\
    \midrule
    % IBN~\cite{pan2018IBN} & 33.85 & 32.30 & 37.75 & 27.90 & - & - & - & -\\
    % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
    % Iternorm~\cite{huang2019Iternorm} & 31.81 & 32.70 & 33.88 & 27.07 & - & - & - & -\\
    % DRPC~\cite{yue2019DRPC} & 37.42 & 32.14 & 34.12 & 28.06\\
    ISW~\cite{choi2021ISW} & 6.32 & 29.97 & 33.02 & 32.56 & 25.47\\
    % GTR~\cite{peng2021GTR} & 37.53 & 33.75 & 34.52 & 28.17\\
    % DIRL~\cite{xu2022dirl} & 41.04 & 39.15 & 41.60 & -\\
    SHADE~\cite{zhao2022shade} & 8.18 & 30.38 & 35.44 & 36.87 & 27.72\\
    % SAN-SAW~\cite{peng2022san-saw} & 39.75 & 37.34 & 41.86 & 30.79 & - & - & - & -\\
    WildNet~\cite{lee2022wildnet} & 8.27 & 30.29 & 36.32 & 35.39 & 27.57\\
    % Pin the memory~\citeyearpar{kim2022pin} & 3.84 & 5.51 & 5.89 & 7.27\\
    SiamDoGe~\cite{wu2022siamdoge} & 10.60 & 30.71 & 35.84 & 36.45 & 28.40\\
    % TLDR~\cite{kim2023TLDR} & 13.13 & 36.02 & \underline{38.89} & \underline{40.58} & 32.16\\
    TLDR (Kim et al.~\citeyear{kim2023TLDR}) & 13.13 & 36.02 & \underline{38.89} & \underline{40.58} & 32.16\\
    % NP~\cite{fan2023NP} & 40.62 & 35.56 & 38.92 & 27.65 & - & - & - & -\\
    % BlindNet~\citeyearpar{ahn2024BlindNet} & 45.72 & 41.32 & 47.08 & 31.39 & - & - & - & -\\
    FAMix~\cite{fahes2024FAMix} & \underline{14.96} & \underline{37.09} & 38.66 & 40.25 & \underline{32.74}\\
    \midrule
    % DIDEX~\citeyearpar{DIDEX} & 52.40 & 40.90 & 49.20 & - & - & - & - & -\\
    % CMFormer~\cite{bi2024CMFormer} & 55.31 & 49.91 & 60.09 & 43.80 & - & - & - & -\\
    % HGFormer~\cite{ding2023hgformer} & - & - & - & -\\
    SCSD (Ours) & \textbf{22.89} & \textbf{52.21} & \textbf{52.37} & \textbf{51.04} & \textbf{44.63}\\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Adverse Condition setting trained on GTAV.} Mean IoU(\%) comparison of different methods with ResNet-50 backbone. }
\label{tab:acdc}
\end{table}

==> section/exp_tab/table_c.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{max width=0.47\textwidth}
\begin{tabular}{c|ccccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{5}{c}{Trained on Cityscapes (C)} \\
    \cmidrule(lr){2-6}
    & $\rightarrow$ B & $\rightarrow$ M & $\rightarrow$ G & $\rightarrow$ S & Avg.\\
    \midrule
    IBN~\cite{pan2018IBN} & 48.56 & 57.04 & 45.06 & 26.14 & 44.20\\
    % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
    Iternorm~\cite{huang2019Iternorm} & 49.23 & 56.26 & 45.73 & 25.98 & 44.30\\
    % DRPC~\cite{yue2019DRPC}& ResNet-50 & 49.86 & 56.34 & 45.62 & 26.58\\
    ISW~\cite{choi2021ISW} & 50.73 & 58.64 & 45.00 & 26.20 & 45.14\\
    % GTR~\cite{peng2021GTR} & 50.75 & 57.16 & 45.79 & 26.47\\
    % DIRL~\cite{xu2022dirl} & 51.80 & - & 46.52 & 26.50\\
    SHADE~\cite{zhao2022shade} & 50.95 & 60.67 & 48.61 & 27.62 & 46.96\\
    SAN-SAW~\cite{peng2022san-saw} & 52.95 & 59.81 & 47.28 & 28.32 & 47.09\\
    % WildNet~\cite{lee2022wildnet} & 50.94 & 58.79 & 47.01 & 27.95\\
    % Pin the memory~\cite{kim2022pin} & 46.78 & 55.10 & - & -\\
    % SiamDoGe~\cite{wu2022siamdoge} & 51.53 & 59.00 & 45.08 & 26.67\\
    % AdvStyle~\cite{zhong2022advstyle} & - & - & - & -\\
    % TLDR~\cite{kim2023TLDR} & - & - & - & -\\
    % PASTA~\cite{2023PASTA} & - & - & - & -\\
    % SPC-Net~\cite{huang2023spc-net} & - & - & - & - & -\\
    % DPCL~\cite{yang2023DPCL} & 52.29 & - & 46.00 & 26.60 & -\\
    DPCL (Yang et al.~\citeyear{yang2023DPCL}) & 52.29 & - & 46.00 & 26.60 & -\\
    HGFormer~\cite{ding2023hgformer} & 51.50 &  61.60 & 50.40 & 30.10 & 48.40\\
    CMFormer$^{\dagger}$(Bi et al.~\citeyear{bi2024CMFormer}) & 53.60 & \textbf{66.00} & \underline{51.70} & \underline{35.90} & \underline{51.80}\\
    BlindNet~\cite{ahn2024BlindNet} & 51.84 & 60.18 & 47.97 & 28.51 & 47.13\\
    FAMix~\cite{fahes2024FAMix} & \underline{54.07} & 58.72 & 45.12 & 32.67 & 47.65\\
    \midrule
    SCSD (Ours) & \textbf{54.63} & \underline{63.85} & \textbf{52.27} & \textbf{41.36} & \textbf{53.03}\\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Single-source setting trained on Cityscapes.} Mean IoU(\%) comparison of different methods with ResNet-50 backbone. ``-'' indicates the metric is not reported or the official source code is not available. ``$\dagger$'' means the method using Swin-T as the backbone.}
\label{tab:c}
\end{table}

==> section/exp_tab/table_g_backup.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{max width=0.47\textwidth}
\begin{tabular}{c|ccccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{5}{c}{Trained on GTAV (G)} \\
    \cmidrule(lr){2-6}
    % \midrule
    & $\rightarrow$C & $\rightarrow$B & $\rightarrow$M & $\rightarrow$S & Avg.\\
    \midrule
    IBN~\cite{pan2018IBN} & 33.85 & 32.30 & 37.75 & 27.90 & 32.95\\
    % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
    Iternorm~\cite{huang2019Iternorm} & 31.81 & 32.70 & 33.88 & 27.07 & 31.37\\
    % DRPC~\cite{yue2019DRPC} & 37.42 & 32.14 & 34.12 & 28.06\\
    ISW~\cite{choi2021ISW} & 36.58 & 35.20 & 40.33 & 28.30 & 35.10\\
    % GTR~\cite{peng2021GTR} & 37.53 & 33.75 & 34.52 & 28.17\\
    % DIRL~\cite{xu2022dirl} & 41.04 & 39.15 & 41.60 & -\\
    SHADE~\cite{zhao2022shade} & 44.65 & 39.28 & 43.34 & 28.41 & 38.92\\
    SAN-SAW~\cite{peng2022san-saw} & 39.75 & 37.34 & 41.86 & 30.79 & 37.44\\
    WildNet~\cite{lee2022wildnet} & 44.62 & 38.42 & 46.09 & 31.34 & 40.12\\
    % Pin the memory~\cite{kim2022pin} & 41.00 & 34.60 & 37.40 & 27.08\\
    % SiamDoGe~\citeyearpar{wu2022siamdoge} & 42.96 & 37.54 & 40.64 & 28.34\\
    % AdvStyle~\citeyearpar{zhong2022advstyle} & 39.62 & 35.54 & 37.00 & -\\
    % TLDR~\cite{kim2023TLDR} & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    TLDR (Kim et al.~\citeyear{kim2023TLDR}) & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    % PASTA~\cite{2023PASTA} & - & - & - & -\\
    % DPCL~\cite{yang2023DPCL} & 44.87 & 40.21 & 46.74 & 26.60 & 39.61\\
    DPCL (Yang et al.~\citeyear{yang2023DPCL}) & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    SPC-Net~\cite{huang2023spc-net} & 44.10 & 40.46 & 45.51 & -& -\\
    % NP~\cite{fan2023NP} & 40.62 & 35.56 & 38.92 & 27.65 & - & - & - & -\\
    BlindNet~\cite{ahn2024BlindNet} & 45.72 & 41.32 & 47.08 & 31.39 & 41.38\\
    FAMix~\cite{fahes2024FAMix} & \underline{48.15} & \textbf{45.61} & \underline{52.11} & \underline{34.23} & \underline{45.03}\\
    % DIDEX$^{*}$~\cite{DIDEX} & \underline{52.40} & 40.90 & 49.20 & - & -\\
    % CMFormer~\citeyearpar{bi2024CMFormer} & 55.31 & 49.91 & 60.09 & 43.80\\
    % HGFormer~\cite{ding2023hgformer} & - & - & - & -\\
    \midrule
    SCSD (Ours) & \textbf{51.72} & \underline{44.67} & \textbf{56.98} & \textbf{43.08} & \textbf{49.11}\\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Single-source setting trained on GTAV.} Mean IoU(\%) comparison of different methods with ResNet-50 backbone. ``-'' indicates the metric is not reported or the official source code is not available. The \textbf{best} and \underline{second best} results are emphasized.}
\label{tab:g}
\end{table}

==> section/exp_tab/table_g_r50x16.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{max width=0.47\textwidth}
\begin{tabular}{c|ccccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{5}{c}{Trained on GTAV (G)} \\
    \cmidrule(lr){2-6}
    % \midrule
    & $\rightarrow$C & $\rightarrow$B & $\rightarrow$M & $\rightarrow$S & Avg.\\
    \midrule
    IBN~\cite{pan2018IBN} & 33.85 & 32.30 & 37.75 & 27.90 & 32.95\\
    % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
    Iternorm~\cite{huang2019Iternorm} & 31.81 & 32.70 & 33.88 & 27.07 & 31.37\\
    % DRPC~\cite{yue2019DRPC} & 37.42 & 32.14 & 34.12 & 28.06\\
    ISW~\cite{choi2021ISW} & 36.58 & 35.20 & 40.33 & 28.30 & 35.10\\
    % GTR~\cite{peng2021GTR} & 37.53 & 33.75 & 34.52 & 28.17\\
    % DIRL~\cite{xu2022dirl} & 41.04 & 39.15 & 41.60 & -\\
    SHADE~\cite{zhao2022shade} & 44.65 & 39.28 & 43.34 & 28.41 & 38.92\\
    SAN-SAW~\cite{peng2022san-saw} & 39.75 & 37.34 & 41.86 & 30.79 & 37.44\\
    WildNet~\cite{lee2022wildnet} & 44.62 & 38.42 & 46.09 & 31.34 & 40.12\\
    % Pin the memory~\cite{kim2022pin} & 41.00 & 34.60 & 37.40 & 27.08\\
    % SiamDoGe~\citeyearpar{wu2022siamdoge} & 42.96 & 37.54 & 40.64 & 28.34\\
    % AdvStyle~\citeyearpar{zhong2022advstyle} & 39.62 & 35.54 & 37.00 & -\\
    % TLDR~\cite{kim2023TLDR} & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    TLDR (Kim et al.~\citeyear{kim2023TLDR}) & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    % PASTA~\cite{2023PASTA} & - & - & - & -\\
    % DPCL~\cite{yang2023DPCL} & 44.87 & 40.21 & 46.74 & 26.60 & 39.61\\
    DPCL (Yang et al.~\citeyear{yang2023DPCL}) & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    SPC-Net~\cite{huang2023spc-net} & 44.10 & 40.46 & 45.51 & -& -\\
    % NP~\cite{fan2023NP} & 40.62 & 35.56 & 38.92 & 27.65 & - & - & - & -\\
    BlindNet~\cite{ahn2024BlindNet} & 45.72 & 41.32 & 47.08 & 31.39 & 41.38\\
    FAMix~\cite{fahes2024FAMix} & 48.15 & \underline{45.61} & \underline{52.11} & \underline{34.23} & \underline{45.03}\\
    DIDEX$^{*}$~\cite{DIDEX} & \underline{52.40} & 40.90 & 49.20 & - & -\\
    % CMFormer~\citeyearpar{bi2024CMFormer} & 55.31 & 49.91 & 60.09 & 43.80\\
    % HGFormer~\cite{ding2023hgformer} & - & - & - & -\\
    \midrule
    SCSD (Ours) & \textbf{55.76} & \textbf{49.05} & \textbf{61.25} & \textbf{46.48} & \textbf{53.14}\\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Single-source setting trained on GTAV.} Mean IoU(\%) comparison of different methods with ResNet-50 backbone. ``-'' indicates the metric is not reported or the official source code is not available. $^{*}$ means the use of additional data. The \textbf{best} and \underline{second best} results are emphasized.}
\label{tab:g}
\end{table}

==> section/exp_tab/table_g_s_r50x16.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{max width=0.47\textwidth}
\begin{tabular}{c|cccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{4}{c}{Trained on Two Datasets (G+S)} \\
    \cmidrule(lr){2-5}
    & $\rightarrow$ C & $\rightarrow$ B & $\rightarrow$ M & Avg.\\
    \midrule
    IBN~\cite{pan2018IBN} & 35.55 & 32.18 & 38.09 & 35.27\\
    ISW~\cite{choi2021ISW} & 37.69 & 34.09 & 38.49 & 36.76\\
    SHADE~\cite{zhao2022shade} & 47.43 & 40.30 & 47.60 & 45.11\\
    % SAN-SAW~\cite{peng2022san-saw} & 52.95 & 59.81 & 47.28 & 28.32\\
    % WildNet~\cite{lee2022wildnet} & 50.94 & 58.79 & 47.01 & 27.95\\
    Pin the memory~\cite{kim2022pin} & 44.51 & 38.07 & 42.70 & 41.76\\
    % SiamDoGe~\cite{wu2022siamdoge} & 51.53 & 59.00 & 45.08 & 26.67\\
    AdvStyle~\cite{zhong2022advstyle} & 39.29 & 39.26 & 41.14 & 39.90\\
    % TLDR~\cite{kim2023TLDR} & 48.83 & 42.58 & 47.80 & 46.40\\
    TLDR (Kim et al.~\citeyear{kim2023TLDR}) & 48.83 & 42.58 & 47.80 & 46.40\\
    % PASTA~\cite{2023PASTA} & - & - & - & -\\
    SPC-Net~\cite{huang2023spc-net} & 46.36 & 43.18 & 48.23 & 45.92\\
    % DPCL~\cite{yang2023DPCL} & 52.29 & - & 46.00 & 26.60\\
    % HGFormer~\cite{ding2023hgformer} & Swin-T & 53.4 & 66.9 & 51.3 & 33.6\\
    % BlindNet~\cite{ahn2024BlindNet} & 51.84 & 60.18 & 47.97 & 28.51\\
    FAMix~\cite{fahes2024FAMix} & \underline{49.41} & \underline{45.51} & \underline{51.61} & \underline{48.84}\\
    % BlindNet~\cite{ahn2024BlindNet} & - & - & - & -\\
    % CMFormer$^{\dag}$~\citeyearpar{bi2024CMFormer} & \textbf{59.70} & 53.36 & 61.61 & 58.22\\
    \midrule
    SCSD (Ours) & \textbf{58.27} & \textbf{50.12} & \textbf{59.04} & \textbf{55.81}\\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Multi-source setting trained on GTAV + SYNTHIA.} Mean IoU(\%) comparison of different methods with ResNet-50 backbone.}
\label{tab:g_s}
\end{table}

==> section/exp_tab/table_main.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{cc}
        \begin{subtable}[t]{0.48\textwidth}
            \centering
            \resizebox{\linewidth}{!}{%
            \begin{Large}
            \begin{tabular}{c|cccc}
                \toprule
                \multirow{2}{*}{Method} & \multicolumn{4}{c}{Trained on GTAV (G)} \\
                \cmidrule(lr){2-5}
                % \midrule
                & $\rightarrow$ C & $\rightarrow$ B & $\rightarrow$ M & $\rightarrow$ S\\
                \midrule
                IBN~\citeyearpar{pan2018IBN} & 33.85 & 32.30 & 37.75 & 27.90\\
                % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
                Iternorm~\citeyearpar{huang2019Iternorm} & 31.81 & 32.70 & 33.88 & 27.07\\
                % DRPC~\cite{yue2019DRPC} & 37.42 & 32.14 & 34.12 & 28.06\\
                ISW~\citeyearpar{choi2021ISW} & 36.58 & 35.20 & 40.33 & 28.30\\
                % GTR~\cite{peng2021GTR} & 37.53 & 33.75 & 34.52 & 28.17\\
                % DIRL~\cite{xu2022dirl} & 41.04 & 39.15 & 41.60 & -\\
                SHADE~\citeyearpar{zhao2022shade} & 44.65 & 39.28 & 43.34 & 28.41\\
                SAN-SAW~\citeyearpar{peng2022san-saw} & 39.75 & 37.34 & 41.86 & 30.79\\
                WildNet~\citeyearpar{lee2022wildnet} & 44.62 & 38.42 & 46.09 & 31.34\\
                % Pin the memory~\cite{kim2022pin} & 41.00 & 34.60 & 37.40 & 27.08\\
                % SiamDoGe~\citeyearpar{wu2022siamdoge} & 42.96 & 37.54 & 40.64 & 28.34\\
                % AdvStyle~\citeyearpar{zhong2022advstyle} & 39.62 & 35.54 & 37.00 & -\\
                TLDR~\citeyearpar{kim2023TLDR} & 46.51 & 42.58 & 46.18 & 30.57\\
                % PASTA~\cite{2023PASTA} & - & - & - & -\\
                DPCL~\citeyearpar{yang2023DPCL} & 44.87 & 40.21 & 46.74 & 26.60\\
                SPC-Net~\citeyearpar{huang2023spc-net} & 44.10 & 40.46 & 45.51 & -\\
                % NP~\cite{fan2023NP} & 40.62 & 35.56 & 38.92 & 27.65 & - & - & - & -\\
                BlindNet~\citeyearpar{ahn2024BlindNet} & 45.72 & 41.32 & 47.08 & 31.39\\
                FAMix~\citeyearpar{fahes2024FAMix} & 48.15 & \underline{45.61} & \underline{52.11} & \underline{34.23}\\
                DIDEX$^{*}$~\citeyearpar{DIDEX} & \underline{52.40} & 40.90 & 49.20 & -\\
                % CMFormer~\citeyearpar{bi2024CMFormer} & 55.31 & 49.91 & 60.09 & 43.80\\
                % HGFormer~\cite{ding2023hgformer} & - & - & - & -\\
                SCSD (Ours) & \textbf{56.22} & \textbf{48.20} & \textbf{59.58} & \textbf{46.20}\\
                \bottomrule
            \end{tabular}
            \end{Large}
            }
            \caption{Single-source DGSS trained on GTAV. Performance of SCSD compared to other DGSS methods trained on C and evaluated on B, M, G and S for ResNet-50 backbone. $^{*}$ indicates the use of extra-data. The \textbf{best} and \underline{second best} results are emphasized.}
            \label{tab:g}
        \end{subtable} &
        
        \begin{subtable}[t]{0.48\textwidth}
            \centering
            \resizebox{\linewidth}{!}{%
            \begin{Large}
            \begin{tabular}{c|cccc}
                \toprule
                \multirow{2}{*}{Method} & \multicolumn{4}{c}{Trained on Cityscapes (C)} \\
                \cmidrule(lr){2-5}
                & $\rightarrow$ B & $\rightarrow$ M & $\rightarrow$ G & $\rightarrow$ S \\
                \midrule
                IBN~\citeyearpar{pan2018IBN} & 48.56 & 57.04 & 45.06 & 26.14\\
                % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
                Iternorm~\citeyearpar{huang2019Iternorm} & 49.23 & 56.26 & 45.73 & 25.98\\
                % DRPC~\cite{yue2019DRPC}& ResNet-50 & 49.86 & 56.34 & 45.62 & 26.58\\
                ISW~\citeyearpar{choi2021ISW} & 50.73 & 58.64 & 45.00 & 26.20\\
                % GTR~\cite{peng2021GTR} & 50.75 & 57.16 & 45.79 & 26.47\\
                % DIRL~\cite{xu2022dirl} & 51.80 & - & 46.52 & 26.50\\
                SHADE~\citeyearpar{zhao2022shade} & 50.95 & 60.67 & 48.61 & 27.62\\
                SAN-SAW~\citeyearpar{peng2022san-saw} & 52.95 & 59.81 & 47.28 & 28.32\\
                % WildNet~\cite{lee2022wildnet} & 50.94 & 58.79 & 47.01 & 27.95\\
                % Pin the memory~\cite{kim2022pin} & 46.78 & 55.10 & - & -\\
                % SiamDoGe~\cite{wu2022siamdoge} & 51.53 & 59.00 & 45.08 & 26.67\\
                % AdvStyle~\cite{zhong2022advstyle} & - & - & - & -\\
                % TLDR~\cite{kim2023TLDR} & - & - & - & -\\
                % PASTA~\cite{2023PASTA} & - & - & - & -\\
                SPC-Net~\citeyearpar{huang2023spc-net} & - & - & - & -\\
                DPCL~\citeyearpar{yang2023DPCL} & 52.29 & - & 46.00 & 26.60\\
                HGFormer~\citeyearpar{ding2023hgformer} & 51.50 &  61.60 & 50.40 & 30.10\\
                CMFormer$^{*}$~\citeyearpar{bi2024CMFormer} & 53.60 & \underline{66.00} & \underline{51.70} & \underline{42.70}\\
                BlindNet~\citeyearpar{ahn2024BlindNet} & 51.84 & 60.18 & 47.97 & 28.51\\
                FAMix~\citeyearpar{fahes2024FAMix} & \underline{54.07} & 58.72 & 45.12 & 32.67\\
                SCSD (Ours) & \textbf{58.36} & \textbf{69.63} & \textbf{56.16} & \textbf{47.67}\\
                \bottomrule
            \end{tabular}
            \end{Large}
            }
            \caption{Single-source DGSS trained on Cityscapes. ``*'' means the results of the same scale backbone are not mentioned in original paper and are obtained by our re-implementation and evaluation. The \textbf{best} and \underline{second best} results are emphasized.}
            \label{tab:c}
        \end{subtable} \\
        
        \begin{subtable}[t]{0.48\textwidth}
            \centering
            \resizebox{\linewidth}{!}{%
            \begin{Large}
            \begin{tabular}{c|cccc}
                \toprule
                \multirow{2}{*}{Method} & \multicolumn{4}{c}{Trained on Two Datasets (G+S)} \\
                \cmidrule(lr){2-5}
                & $\rightarrow$ C & $\rightarrow$ B & $\rightarrow$ M & Mean\\
                \midrule
                IBN~\citeyearpar{pan2018IBN} & 35.55 & 32.18 & 38.09 & 35.27\\
                ISW~\citeyearpar{choi2021ISW} & 37.69 & 34.09 & 38.49 & 36.76\\
                SHADE~\citeyearpar{zhao2022shade} & 47.43 & 40.30 & 47.60 & 45.11\\
                % SAN-SAW~\cite{peng2022san-saw} & 52.95 & 59.81 & 47.28 & 28.32\\
                % WildNet~\cite{lee2022wildnet} & 50.94 & 58.79 & 47.01 & 27.95\\
                Pin the memory~\citeyearpar{kim2022pin} & 44.51 & 38.07 & 42.70 & 41.76\\
                % SiamDoGe~\cite{wu2022siamdoge} & 51.53 & 59.00 & 45.08 & 26.67\\
                AdvStyle~\citeyearpar{zhong2022advstyle} & 39.29 & 39.26 & 41.14 & 39.90\\
                TLDR~\citeyearpar{kim2023TLDR} & 48.83 & 42.58 & 47.80 & 46.40\\
                % PASTA~\cite{2023PASTA} & - & - & - & -\\
                SPC-Net~\citeyearpar{huang2023spc-net} & 46.36 & 43.18 & 48.23 & 45.92\\
                % DPCL~\cite{yang2023DPCL} & 52.29 & - & 46.00 & 26.60\\
                % HGFormer~\cite{ding2023hgformer} & Swin-T & 53.4 & 66.9 & 51.3 & 33.6\\
                % BlindNet~\cite{ahn2024BlindNet} & 51.84 & 60.18 & 47.97 & 28.51\\
                FAMix~\citeyearpar{fahes2024FAMix} & 49.41 & 45.51 & 51.61 & 48.84\\
                BlindNet~\citeyearpar{ahn2024BlindNet} & - & - & - & -\\
                % CMFormer$^{\dag}$~\citeyearpar{bi2024CMFormer} & \textbf{59.70} & 53.36 & 61.61 & 58.22\\
                SCSD (Ours) & 56.90 & \textbf{49.53} & \textbf{-} & \textbf{-}\\
                \bottomrule
            \end{tabular}
            \end{Large}
            }
            \caption{Multi-source DGSS trained on GTAV + SYNTHIA. ``\(\dag\)'' denotes}
            \label{tab:g_s}
        \end{subtable} &
        
        \begin{subtable}[t]{0.48\textwidth}
            \centering
            \resizebox{\linewidth}{!}{%
            \begin{Large}
            \begin{tabular}{c|cccc}
                \toprule
                \multirow{2}{*}{Method} & \multicolumn{4}{c}{Trained on GTAV (G)} \\
                \cmidrule(lr){2-5}
                % \midrule
                & $\rightarrow$ AN & $\rightarrow$ AS & $\rightarrow$ AR & $\rightarrow$ AF\\
                \midrule
                % IBN~\cite{pan2018IBN} & 33.85 & 32.30 & 37.75 & 27.90 & - & - & - & -\\
                % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
                % Iternorm~\cite{huang2019Iternorm} & 31.81 & 32.70 & 33.88 & 27.07 & - & - & - & -\\
                % DRPC~\cite{yue2019DRPC} & 37.42 & 32.14 & 34.12 & 28.06\\
                ISW~\citeyearpar{choi2021ISW} & 6.32 & 29.97 & 33.02 & 32.56\\
                % GTR~\cite{peng2021GTR} & 37.53 & 33.75 & 34.52 & 28.17\\
                % DIRL~\cite{xu2022dirl} & 41.04 & 39.15 & 41.60 & -\\
                SHADE~\citeyearpar{zhao2022shade} & 8.18 & 30.38 & 35.44 & 36.87\\
                % SAN-SAW~\cite{peng2022san-saw} & 39.75 & 37.34 & 41.86 & 30.79 & - & - & - & -\\
                WildNet~\citeyearpar{lee2022wildnet} & 8.27 & 30.29 & 36.32 & 35.39\\
                % Pin the memory~\citeyearpar{kim2022pin} & 3.84 & 5.51 & 5.89 & 7.27\\
                SiamDoGe~\citeyearpar{wu2022siamdoge} & 10.60 & 30.71 & 35.84 & 36.45\\
                TLDR~\citeyearpar{kim2023TLDR} & 13.13 & 36.02 & \underline{38.89} & \underline{40.58}\\
                % NP~\cite{fan2023NP} & 40.62 & 35.56 & 38.92 & 27.65 & - & - & - & -\\
                % BlindNet~\citeyearpar{ahn2024BlindNet} & 45.72 & 41.32 & 47.08 & 31.39 & - & - & - & -\\
                FAMix~\citeyearpar{fahes2024FAMix} & \underline{14.96} & \underline{37.09} & 38.66 & 40.25\\
                % DIDEX~\citeyearpar{DIDEX} & 52.40 & 40.90 & 49.20 & - & - & - & - & -\\
                % CMFormer~\cite{bi2024CMFormer} & 55.31 & 49.91 & 60.09 & 43.80 & - & - & - & -\\
                % HGFormer~\cite{ding2023hgformer} & - & - & - & -\\
                SCSD (Ours) & \textbf{24.27} & \textbf{51.00} & \textbf{50.18} & \textbf{51.02}\\
                \bottomrule
            \end{tabular}
            \end{Large}
            }
            \caption{Adverse Condition DGSS trained on GTAV. We emphasize \textbf{best} and \underline{second best} results.}
            \label{tab:acdc}
        \end{subtable} \\
    \end{tabular}
    \caption{Combined Results of Multiple Tables}
    \label{tab:sota}
\end{table*}


==> supple/table/table_s.tex <==
\begin{table}[!htp]
\centering
\begin{adjustbox}{max width=0.47\textwidth}
\begin{tabular}{c|ccccc}
    \toprule
    \multirow{2.5}{*}{Method} & \multicolumn{5}{c}{Trained on SYNTHIA (S)} \\
    \cmidrule(lr){2-6}
    % \midrule
    & $\rightarrow$C & $\rightarrow$B & $\rightarrow$M & $\rightarrow$G & Avg.\\
    \midrule
    IBN~\cite{pan2018IBN} & 32.04 & 30.57 & 32.16 & 26.90 & 30.92\\
    IW~\cite{pan2018SW} & 28.16 & 27.12 & 26.31 & 26.51 & 27.03\\
    % Iternorm~\cite{huang2019Iternorm} & 31.81 & 32.70 & 33.88 & 27.07 & 31.37\\
    DRPC~\cite{yue2019DRPC} & 35.65 & 31.53 & 32.74 & 28.75 & 32.17\\
    ISW~\cite{choi2021ISW} & 35.83 & 31.62 & 30.84 & 27.68 & 31.99\\
    GTR~\cite{peng2021GTR} & 36.84 & 32.02 & 32.89 & 28.02 & 32.94\\
    % DIRL~\cite{xu2022dirl} & 41.04 & 39.15 & 41.60 & -\\
    % SHADE~\cite{zhao2022shade} & 44.65 & 39.28 & 43.34 & 28.41 & 38.92\\
    SAN-SAW~\cite{peng2022san-saw} & \underline{38.92} & \textbf{35.24} & \underline{34.52} & \underline{29.16} & \underline{34.46}\\
    % WildNet~\cite{lee2022wildnet} & 44.62 & 38.42 & 46.09 & 31.34 & 40.12\\
    % Pin the memory~\cite{kim2022pin} & 41.00 & 34.60 & 37.40 & 27.08\\
    % SiamDoGe~\citeyearpar{wu2022siamdoge} & 42.96 & 37.54 & 40.64 & 28.34\\
    AdvStyle~\citeyearpar{zhong2022advstyle} & 37.59 & 27.45 & 31.76 & - & -\\
    % TLDR~\cite{kim2023TLDR} & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    % TLDR (Kim et al.~\citeyear{kim2023TLDR}) & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    % PASTA~\cite{2023PASTA} & - & - & - & -\\
    % DPCL~\cite{yang2023DPCL} & 44.87 & 40.21 & 46.74 & 26.60 & 39.61\\
    % DPCL (Yang et al.~\citeyear{yang2023DPCL}) & 46.51 & 42.58 & 46.18 & 30.57 & 41.46\\
    % SPC-Net~\cite{huang2023spc-net} & 44.10 & 40.46 & 45.51 & -& -\\
    % NP~\cite{fan2023NP} & 40.62 & 35.56 & 38.92 & 27.65 & - & - & - & -\\
    % BlindNet~\cite{ahn2024BlindNet} & 45.72 & 41.32 & 47.08 & 31.39 & 41.38\\
    % FAMix~\cite{fahes2024FAMix} & 48.15 & \underline{45.61} & \underline{52.11} & \underline{34.23} & \underline{45.03}\\
    % DIDEX$^{*}$~\cite{DIDEX} & \underline{52.40} & 40.90 & 49.20 & - & -\\
    % CMFormer$^{\dagger}$(Bi et al.~\citeyear{bi2024CMFormer}) & 44.59 & 33.44 & 43.25 & 40.65 & -\\
    % HGFormer~\cite{ding2023hgformer} & - & - & - & -\\
    \midrule
    SCSD (Ours) & \textbf{40.40} & \underline{32.19} & \textbf{38.70} & \textbf{37.64} & \textbf{37.23}\\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Single-source setting trained on SYNTHIA.} Mean IoU(\%) comparison of different methods with ResNet-50 backbone. ``-'' indicates the metric is not reported or the official source code is not available. The \textbf{best} and \underline{second best} results are emphasized.}
\label{tab:s}
\end{table}


%%%%%%%%%%%%
% \begin{table}[!htp]
% \setlength\tabcolsep{1.5pt} % 调整列间距
% \centering
% \small
% \scriptsize
% \renewcommand{\arraystretch}{0.8}
% \begin{tabular}{c|cccccccc}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{8}{c}{Trained on GTAV (G)} \\
%     \cmidrule(lr){2-9}
%     % \midrule
%     & C & B & M & S & AN & AS & AR & AF\\
%     \midrule
%     IBN~\cite{pan2018IBN} & 33.85 & 32.30 & 37.75 & 27.90 & - & - & - & -\\
%     % IW~\cite{} & 48.49 & 55.82 & 44.87 & 26.10\\
%     Iternorm~\cite{huang2019Iternorm} & 31.81 & 32.70 & 33.88 & 27.07 & - & - & - & -\\
%     % DRPC~\cite{yue2019DRPC} & 37.42 & 32.14 & 34.12 & 28.06\\
%     ISW~\cite{choi2021ISW} & 36.58 & 35.20 & 40.33 & 28.30 & 6.32 & 29.97 & 33.02 & 32.56\\
%     % GTR~\cite{peng2021GTR} & 37.53 & 33.75 & 34.52 & 28.17\\
%     % DIRL~\cite{xu2022dirl} & 41.04 & 39.15 & 41.60 & -\\
%     SHADE~\cite{zhao2022shade} & 44.65 & 39.28 & 43.34 & 28.41 & 8.18 & 30.38 & 35.44 & 36.87\\
%     SAN-SAW~\cite{peng2022san-saw} & 39.75 & 37.34 & 41.86 & 30.79 & - & - & - & -\\
%     WildNet~\cite{lee2022wildnet} & 44.62 & 38.42 & 46.09 & 31.34 & 8.27 & 30.29 & 36.32 & 35.39\\
%     Pin the memory~\cite{kim2022pin} & 41.00 & 34.60 & 37.40 & 27.08 & 3.84 & 5.51 & 5.89 & 7.27\\
%     SiamDoGe~\cite{wu2022siamdoge} & 42.96 & 37.54 & 40.64 & 28.34 & 10.60 & 30.71 & 35.84 & 36.45\\
%     AdvStyle~\cite{zhong2022advstyle} & 39.62 & 35.54 & 37.00 & - & - & - & - & -\\
%     TLDR~\cite{kim2023TLDR} & 46.51 & 42.58 & 46.18 & 30.57 & 13.13 & 36.02 & 38.89 & 40.58\\
%     % PASTA~\cite{2023PASTA} & - & - & - & -\\
%     DPCL~\cite{yang2023DPCL} & 44.87 & 40.21 & 46.74 & 26.60 & - & - & - & -\\
%     SPC-Net~\cite{huang2023spc-net} & 44.10 & 40.46 & 45.51 & - & - & - & -\\
%     % NP~\cite{fan2023NP} & 40.62 & 35.56 & 38.92 & 27.65 & - & - & - & -\\
%     BlindNet~\cite{ahn2024BlindNet} & 45.72 & 41.32 & 47.08 & 31.39 & - & - & - & -\\
%     FAMix~\cite{fahes2024FAMix} & 48.15 & 45.61 & 52.11 & 34.23 & 14.96 & 37.09 & 38.66 & 40.25\\
%     DIDEX~\cite{DIDEX} & 52.40 & 40.90 & 49.20 & - & - & - & - & -\\
%     CMFormer~\cite{bi2024CMFormer} & 55.31 & 49.91 & 60.09 & 43.80 & - & - & - & -\\
%     % HGFormer~\cite{ding2023hgformer} & - & - & - & -\\
%     Ours & \textbf{59.0} & \textbf{49.1} & \textbf{-} & \textbf{50.3}\\
%     \bottomrule
% \end{tabular}
% \caption{Single-source DGSS trained on GTAV.}
% \label{table2}
% \end{table}
